High-Dimensional Expanders from Expanders

We present an elementary way to transform an expander graph into a simplicial complex where all high order random walks have a constant spectral gap, i.e., they converge rapidly to the stationary distribution. As an upshot, we obtain new constructions, as well as a natural probabilistic model to sample constant degree high-dimensional expanders. In particular, we show that given an expander graph $G$, adding self loops to $G$ and taking the tensor product of the modified graph with a high-dimensional expander produces a new high-dimensional expander. Our proof of rapid mixing of high order random walks is based on the decomposable Markov chains framework introduced by Jerrum et al.

==> old-stuff.tex <==
\section{XXXXX Beginning of old writing}

\subsubsection{Related Expander Graph Constructions}
(Cite Salil Vadhan's book chapter for this)
\begin{itemize}
    \item Graph tensor product: given $G$, $H$, where $G$ is a $(n_1, d_1, \gamma_1 = 1 - \lambda_1)$ expander and $H$ is a $(n_2, d_2, \gamma_2 = 1 - \lambda_2)$ expander, the graph tensor $G \tensor H$ (take the graph from $A_G \tensor A_H$) is a $(n_1n_2, d_1d_2, \min\{\gamma_1, \gamma_2\})$ expander. 
    
    \item Replacement product: given $G$, $H$, where $G$ is a $(n, d_1, \gamma_1)$ expander and $H$ is a $(d_1, d_2, \gamma_2)$ expander, the replacement product $G \rep H$ is a $(nd_1, 2d_2, \frac{\gamma_1\gamma_2}{16})$ expander. (Reference for this result, according to Theory Toolkit notes: M. Jerrum, J. Son, P. Tetali, and E. Vigoda. Elementary bounds on Poincare and log-Sobolev constants for decomposable Markov chains. Ann. Appl. Probab., 14(4):1741–1765, 2004.) 
    
    \item Zig-zag product: given $G$, $H$, where $G$ is a $(n, d_1, \lambda_1)$ expander and $H$ is a $(d_1, d_2, \lambda_2)$ expander, the zig-zag product $G \zig H$ is a $(n_1, d_1, d_2^2, \gamma_1 \cdot \gamma_2^2)$ expander.
\end{itemize}

\subsubsection{Related Structures}

\begin{itemize}
    \item There are also quantum HDX. See paper ``Efficient quantum tensor product expanders and unitary t-designs via the zigzag product.'' Pranab Sen uses the zig zag product of a quantum HDX and a quantum $t$-tensor product expander of low degree to get a high dimensional quantum $t$-tensor product expander of low degree. 
\end{itemize}

General idea to convey: These constructions try to combine the best attributes of two different expanders into one expander. 

\subsection{Local Expansion and Mixing Time}

Many applications of expander graphs stem from the fact that random walks on expanders mix rapidly. An analogue of this property in the high dimensional setting deals with random walks over hyperedges, rather than just random walks over vertices. 

Let $X$ be a degree $d$ high dimensional expander, and let $X(k)$ be the set of all size $k$ hyperedges in $X$, where $1 \leq k \leq d$. Construct bipartite graph $H$ over vertices $X(k) \cup X(k + 1)$. The only edges in $H$ are between $X(k)$ and $X(k + 1)$. Furthermore, assign each element $T \in X(k + 1)$ some weight $w(T)$. Consider the following random walk transitions:
\begin{itemize}
    \item At an element $T \in X(k + 1)$, transition to $S \in X(k)$ with probability $\frac{1}{k + 1}$ if $S \subset T$. 
    
    \item At an element $S \in X(k)$, transition to $T \in X(k + 1)$ with probability $\frac{w(T)}{\sum_{T \in X(k + 1): T \supset S} w(T)}$. 
\end{itemize}
If we restrict the walk above only to the elements of $X(k)$, we call this the ``up-down'' walk, and its transition matrix is specified by $P_k^\land$. Similarly, if we restrict the walk only to the elements of $X(k + 1)$, we call this the ``down-up'' walk, and specify its transition matrix by $P_{k + 1}^\lor$. The relationship between local expansion and fast mixing of these walks is quantified by the following theorems:
TODO: INSERT KO THEOREM HERE. 

\section{Up-down random walks}

\begin{theorem}\label{thm:up-down random walk spectral gap}
    Let $G$ be a triangle free $\dT$--regular graph with spectral gap $\lambda$ and $\SimpComp$ be a pure $\dH$-dimensional simplicial complex. If the up-down random walk graph on the $k$-faces of $\SimpComp$ is $f$-regular and has spectral gap $\gamma$. Then up-down random walk on the $k$-faces of the local densifier $\LD(G,\SimpComp)$ has spectral gap at least $\min( ? , ?)$.
\end{theorem}

For a given graph $G$ we provide a way to construct a graph $G_\ell$ which will be a useful class of graphs in our analysis of the the up-down random walks on $\LD(G,\SimpComp)$. 
 First, construct a graph $\hat{G}_{\ell}$: 
\begin{enumerate}
    \item vertex set equal to $E(G)\times V(\text{Hypercube}(\ell))$, and
    \item edge set equal to $\{ \{(e,v_1),(e,v_2)\} : e \in E(G), (v_1,v_2)\in E(\text{Hypercube}(\ell))\}$.
    \item for every $e \in E(G)$ sample a random order on the two end points so that $e$ becomes an ordered pair $(e(0),e(1))$. For every vertex $u\in V(G)$, merge the vertices $\{(e,v) : u = e(b) \text{ and } v = b^{\ell}\}$ into one vertex and denote it $\hat{u}$.
\end{enumerate}

\begin{lemma}\label{lmm:cartesian decomposition}
    Use $\LD(G,\SimpComp)_k$ to denote the up-down random walk on the $k$-faces of the local densifier. $\LD(G,\SimpComp)_k$ is the Cartesian product graph of $\SimpComp_k$, the $k$-up random walk graph on $\SimpComp$, and the graph $\hat{G}_{k+1}$ with the following edge weights: every $\hat{u}$ has a self-loop of weight $\frac{1}{f+(k+1)\dT}$ and other outgoing edges each of weight $\frac{1}{f+(k+1)\dT}$; every $(e,v)$ has a self-loop of weight $\frac{1}{f+k+1}$ and other outgoing edges each of weight $\frac{1}{f+k+1}$.
\end{lemma}

\begin{lemma}\label{lmm:reduce to f graph}
    If $\SimpComp_k$ is $f$-regular, then for every eigenvalue $\lambda$ of $\LD(G,\SimpComp)_k$'s transitional matrix is also an eigenvalue of the transitional matrix of the graph $\hat{G}_{k+1}$, and the edges of $\hat{G}$ are weighted in the following way: every $\hat{u}$ has a self-loop of weight $\frac{f}{f+(k+1)\dT}$ and other outgoing edges each of weight $\frac{1}{f+(k+1)\dT}$; every $(e,v)$ has a self-loop of weight $\frac{f}{f+k+1}$ and other outgoing edges each of weight $\frac{1}{f+k+1}$.
\end{lemma}

\begin{proof}
    The vertex set $V(\LD(G,\SimpComp)_k) = V(\SimpComp_k) \times V(\hat{G})$. If $\lambda$ is an eigenvalue of the transitional matrix of $\LD(G,\SimpComp)_k$, let $\vec{w}$ be a corresponding eigenvector. Use $w(s,u)$ to denote the weight of a vertex $(s,u)$ in $\vec{w}$. Then $\lambda$ is also an eigenvalue of $\hat{G}$ with a corresponding eigenvector $\vec{\hat{w}}$. The entries of $\vec{\hat{w}}$ is defined as  $\hat{w}(u) = \sum_{s\in V(\SimpComp_k)} w(s,u)$ for every vertex $u\in V(\hat{G})$. We verify that $\vec{\hat{w}}$ is indeed an eigenvector with eigenvalue $\lambda$. If $u_1$ is a vertex of the form $\hat{u}$:
    \begin{align*}
        \left(A_{\hat{G}}\vec{\hat{w}}\right)_{u_1} 
        &= \frac{f}{f+(k+1)\dT}\hat{w}(u_1) + \sum_{u_2\in N_{\hat{G}}(u_1)}\frac{1}{f+k+1}\hat{w}(u_2) \\
        &= f\sum_{s_1\in V(\SimpComp_k)}\frac{1}{f+(k+1)\dT}w(s_1,u_1) + \sum_{s_1\in V(\SimpComp_k)}\sum_{u_2\in N_{\hat{G}}(u_1)}\frac{1}{f+k+1}w(s_1,u_2)  \\ 
        &= \sum_{s_1\in V(\SimpComp_k)}\left( \sum_{s_2\in N_{\SimpComp_k}(s_1)} \frac{1}{f+(k+1)\dT}w(s_2,u_1) + \sum_{u_2\in N_{\hat{G}}(u_1)}\frac{1}{f+k+1}w(s_1,u_2) \right) \\
        &= \sum_{s_1\in V(\SimpComp_k)} \lambda w(s_1,u_1) \\
        &= \lambda\hat{w}(u_1)
    \end{align*}
    The other case can be verified in the same way.
\end{proof}


% Roadmap:
% \begin{enumerate}
%     \item Intro: def lambda hdx (mention other definitions); Ramanujan complexes + KO construction (their expansions + degree); the challenge of coming up with probabilistic construction (need roughly $\left(\frac{\log{n}}{n}\right)^{1/h}$-degree Erdos-Renyi graph to make $(h-2)$-links connected); then technical overview (brag a bit, mention the construction is strongly explicit, probabilistic construction, combinatorial...); applications of hdx.
%     \item Preliminaries 
%     \item Construction of local densifier (vaguely resembles zig-zag but not independent sets + matching). Analysis of local and global expansions.(mention the construction is strongly explicit) [Sidhanth]
%     \item Up-down walks.
%     \item Further directions: for local densifier: improve the local expansion beyond 1/2; is there a Alon-Boppana bound for hdx (i.e. given degree and dimension, what's the best local-spectral hdx you can get).[Elizabeth]
% \end{enumerate}
